AUEditNet: Dual-Branch Facial Action Unit Intensity Manipulation with Implicit Disentanglement

Facial action unit (AU) intensity plays a pivotal role in quantifying fine-grained expression behaviors, which is an effective condition for facial expression manipulation. However, publicly available datasets containing intensity annotations for multiple AUs remain severely limited, often featuring a restricted number of subjects. This limitation places challenges to the AU intensity manipulation in images due to disentanglement issues, leading researchers to resort to other large datasets with pretrained AU intensity estimators for pseudo labels. In addressing this constraint and fully leveraging manual annotations of AU intensities for precise manipulation, we introduce AUEditNet. Our proposed model achieves impressive intensity manipulation across 12 AUs, trained effectively with only 18 subjects. Utilizing a dual-branch architecture, our approach achieves comprehensive disentanglement of facial attributes and identity without necessitating additional loss functions or implementing with large batch sizes. This approach offers a potential solution to achieve desired facial attribute editing despite the dataset's limited subject count. Our experiments demonstrate AUEditNet's superior accuracy in editing AU intensities, affirming its capability in disentangling facial attributes and identity within a limited subject pool. AUEditNet allows conditioning by either intensity values or target images, eliminating the need for constructing AU combinations for specific facial expression synthesis. Moreover, AU intensity estimation, as a downstream task, validates the consistency between real and edited images, confirming the effectiveness of our proposed AU intensity manipulation method.

==> figures/fig-celeba_single_au-two_cols.tex <==
\begin{figure*}
    \captionsetup[subfigure]{labelformat=empty}
    \captionsetup[subfigure]{justification=centering}
    \centering
        \begin{minipage}{0.3cm}
        \rotatebox{90}{\scriptsize{AU $5$  ~~~~~~~~~~~~~~~~~~ AU $4$ ~~~~~~~~~~~~~~~~~~ AU $2$ ~~~~~~}}
        \end{minipage}%
    \begin{subfigure}[t]{0.099\linewidth}
        \begin{minipage}{1\linewidth}
        \caption{Inversion}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00046_inverted.jpg}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00029_inverted.jpg}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00012_inverted.jpg}
        \end{minipage}
    \label{fig:comp_input0}
  \end{subfigure}
  \hspace{-0.015\linewidth}
  \centering
    \begin{subfigure}[t]{0.099\linewidth}
        \begin{minipage}{1\linewidth}
        \caption{$a_{tar} = 0$}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00046_0.jpg}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00029_4.jpg}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00012_8.jpg}
        \end{minipage}
    \label{fig:comp_inver0}
  \end{subfigure}
  \hspace{-0.015\linewidth}
  \centering
    \begin{subfigure}[t]{0.099\linewidth}
        \begin{minipage}{1\linewidth}
        \caption{$a_{tar} = 2$}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00046_1.jpg}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00029_5.jpg}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00012_9.jpg}
        \end{minipage}
    \label{fig:comp_redir0}
  \end{subfigure}
  \hspace{-0.015\linewidth}
  \centering
    \begin{subfigure}[t]{0.099\linewidth}
        \begin{minipage}{1\linewidth}
        \caption{$a_{tar} = 4$}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00046_2.jpg}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00029_6.jpg}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00012_10.jpg}
        \end{minipage}
    \label{fig:comp_tar0}
  \end{subfigure}
  \hspace{-0.008\linewidth}
  \centering
    \begin{subfigure}[t]{0.099\linewidth}
        \begin{minipage}{1\linewidth}
        \caption{$a_{tar} = -2$}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00046_3.jpg}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00029_7.jpg}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00012_11.jpg}
        \end{minipage}
    \label{fig:comp_input1}
  \end{subfigure}
    \begin{minipage}{0.3cm}
        \rotatebox{90}{\scriptsize{AU $25$ ~~~~~~~~~~~~~~~~ AU $15$ ~~~~~~~~~~~~~~~~~ AU $6$ ~~~~~~}}
    \end{minipage}%
    \begin{subfigure}[t]{0.099\linewidth}
        \begin{minipage}{1\linewidth}
        \caption{Inversion}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00021_inverted.jpg}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00006_inverted.jpg}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00053_inverted.jpg}
        \end{minipage}
    \label{fig:comp_input2}
  \end{subfigure}
  \hspace{-0.015\linewidth}
  \centering
    \begin{subfigure}[t]{0.099\linewidth}
        \begin{minipage}{1\linewidth}
        \caption{$a_{tar} = 0$}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00021_12.jpg}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00006_16.jpg}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00053_20.jpg}
        \end{minipage}
    \label{fig:comp_inver1}
  \end{subfigure}
  \hspace{-0.015\linewidth}
  \centering
    \begin{subfigure}[t]{0.099\linewidth}
        \begin{minipage}{1\linewidth}
        \caption{$a_{tar} = 2$}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00021_13.jpg}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00006_17.jpg}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00053_21.jpg}
        \end{minipage}
    \label{fig:comp_redir1}
  \end{subfigure}
  \hspace{-0.015\linewidth}
  \centering
    \begin{subfigure}[t]{0.099\linewidth}
        \begin{minipage}{1\linewidth}
        \caption{$a_{tar} = 4$}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00021_14.jpg}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00006_18.jpg}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00053_22.jpg}
        \end{minipage}
    \label{fig:comp_tar1}
  \end{subfigure}
  \hspace{-0.008\linewidth}
  \centering
    \begin{subfigure}[t]{0.099\linewidth}
        \begin{minipage}{1\linewidth}
        \caption{$a_{tar} = -2$}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00021_15.jpg}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00006_19.jpg}
        \includegraphics[width=1\linewidth]{figs/celeba_single_au/00053_23.jpg}
        \end{minipage}
    \label{fig:comp_input3}
  \end{subfigure}
  \caption{Qualitatively comparisons between ST-ED and ReDirTrans-GAN. Red boxes represent different face covering ranges.} 
  \label{fig:red_comparison}
\end{figure*}

==> figures/fig-data_augmentation.tex <==
\begin{figure}  
\begin{center}  
    \includegraphics[width=0.88\linewidth]{figs/aug.pdf}
    \caption{Synthetic data augmentation via AUEditNet for the AU intensity estimation task. `Raw' denotes training with real data only. `Aug' denotes training with both real and synthetic data. `Fully Supervised' denotes the baseline with using all training samples of the DISFA training dataset. } 
    \label{fig:data_aug}
\end{center} 
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/supptab-icc_inversion_four_methods.tex <==
\begin{table*}[t]
\centering
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{@{}clccccccccccccc@{}}
\toprule
         &
  Method &
  AU1 &
  AU2 &
  AU4 &
  AU5 &
  AU6 &
  AU9 &
  AU12 &
  AU15 &
  AU17 &
  AU20 &
  AU25 &
  AU26 &
  Avg \\ \midrule \midrule
\multirow{4}{*}{\rotatebox{90}{ICC $(\uparrow)$}} &
  ReDirTrans \cite{jin2023redirtrans} &
  .856 &
  \textbf{.631} &
  .851 &
  .436 &
  .634 &
  .278 &
  .862 &
  .364 &
  .602 &
  .481 &
  .927 &
  .480 &
  .617 \\
 &
 ReDirTrans (\textit{Inv}) &
  \textbf{.858} &
  .623 &
  .873 &
  .437 &
  \textbf{.643} &
  \textbf{.284} &
  .860 &
  \textbf{.371} &
  .619 &
  .488 &
  .930 &
  .464 &
  .621
  \\
 &
  AUEditNet &
  .848 &
  .559 &
  .874 &
  \textbf{.600} &
  .577 &
  .230 &
  \textbf{.890} &
  .276 &
  .669 &
  .511 &
  \textbf{.950} &
  \textbf{.548} &
  .628 \\
  &
  AUEditNet (\textit{Inv}) &
  .853 &
  .551 & 
  \textbf{.885} &
  \textbf{.600} &
  .586 &
  .235 &
  .888 & 
  .283 &
  \textbf{.685} &
  \textbf{.514} &
  .948 &
  .533 &
  \textbf{.631}
   \\ 
   \midrule
\multirow{4}{*}{\rotatebox{90}{MSE $(\downarrow)$}} &
  ReDirTrans \cite{jin2023redirtrans} &
  \textbf{.181} &
  .397 &
  .341 &
  .034 &
  .453 &
  .552 &
  .286 &
  .070 &
  .225 &
  .333 &
  .247 &
  .367 &
  .290 \\
 &
 ReDirTrans (\textit{Inv}) &
  \textbf{.181} &
  .405 &
  .301 & 
  .035 &
  .444 &
  .548 &
  .290 &
  .069 &
  .217 &
  .328 &
  .236 &
  .377 &
  .286
   \\
 &
  AUEditNet &
  .191 &
  .445 &
  .309 &
  .029 &
  .492 &
  .579 &
  .228 &
  .080 &
  .188 &
  .322 &
  .169 &
  .367 &
  .283 \\
  &
  AUEditNet (\textit{Inv}) &
  .186 &
  .452 &
  .291 &
  .030 &
  .483 &
  .574 &
  .230 &
  .080 &
  .181 &
  .321 &
  .171 &
  .377 &
  .281
  \\ \bottomrule
\end{tabular}}
\caption{Comparison to the state-of-the-art action unit (AU) intensity estimation and editing methods in DISFA \cite{mavadati2013disfa}. 
}
\label{supptab:icc_inversion_4}
\end{table*}

==> tables/tab-disfa_all_criteria.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\underline}{\ul}{}
\begin{table*}[t]
\centering
\begin{tabular}{@{}ccccccccccc@{}}
\toprule
 &
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Conditions\\ (Intensity)\end{tabular}}} &
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Image\\ Category\end{tabular}}} &
  \multirow{2}{*}{} &
  \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Image\\ Similarity\end{tabular}}} &
   &
  \textbf{\begin{tabular}[c]{@{}c@{}}Identity\\ Preservation\end{tabular}} &
   &
  \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Editing\\ Accuracy\end{tabular}}} \\ \cmidrule(lr){5-6} \cmidrule(lr){8-8} \cmidrule(l){10-11} 
 &
   &
   &
   &
  L2 $(\downarrow)$ &
  LPIPS $(\downarrow)$ &
   &
  Distance $(\downarrow)$ &
   &
  MSE $(\downarrow)$ &
  ICC(3, 1) $(\uparrow)$ \\ \midrule
\multirow{4}{*}{DeltaEdit \cite{lyu2023deltaedit}} &
  \multirow{2}{*}{Target} &
  Real &
   &
  \textbf{0.022} &
  \textbf{0.165} &
   &
  \textbf{0.396} &
   &
  0.560 &
  0.180 \\
 &
   &
  Inverted &
   &
  \textbf{0.011} &
  \textbf{0.074} &
   &
  \textbf{0.309} &
   &
  0.557 &
  0.194 \\ \cmidrule(l){2-11} 
 &
  \multirow{2}{*}{Zero} &
  Real &
   &
  - &
  - &
   &
  - &
   &
  - &
  - \\
 &
   &
  Inverted &
   &
  - &
  - &
   &
  - &
   &
  - &
  - \\ \midrule
\multirow{4}{*}{ReDirTrans \cite{jin2023redirtrans}} &
  \multirow{2}{*}{Target} &
  Real &
   &
  \textbf{0.022} &
  {\underline{0.169}} &
   &
  0.529 &
   &
  {\underline{ 0.290}} &
  {\underline{ 0.617}} \\
 &
   &
  Inverted &
   &
  0.017 &
  0.137 &
   &
  0.551 &
   &
  {\underline {0.286}} &
  {\underline {0.621}} \\ \cmidrule(l){2-11} 
 &
  \multirow{2}{*}{Zero} &
  Real &
   &
  {\underline {0.026}} &
  {\underline {0.172}} &
   &
  0.600 &
   &
  0.816 &
  - \\
 &
   &
  Inverted &
   &
  {\underline {0.012}} &
  {\underline {0.085}} &
   &
  0.646 &
   &
  0.807 &
  - \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}AUEditNet\\ (Ours)\end{tabular}} &
  \multirow{2}{*}{Target} &
  Real &
   &
  {\underline {0.026}} &
  0.174 &
   &
  {\underline {0.468}} &
   &
  \textbf{0.283} &
  \textbf{0.628} \\
 &
   &
  Inverted &
   &
  {\underline {0.016}} &
  {\underline {0.126}} &
   &
  {\underline {0.435}} &
   &
  \textbf{0.281} &
  \textbf{0.630} \\ \cmidrule(l){2-11} 
 &
  \multirow{2}{*}{Zero} &
  Real &
   &
  {\underline {0.026}} &
  0.179 &
   &
  \textbf{0.426} &
   &
  \textbf{0.102} &
  - \\
 &
   &
  Inverted &
   &
  0.016 &
  0.098 &
   &
  \textbf{0.383} &
   &
  \textbf{0.100} &
  - \\ \bottomrule
\end{tabular}
\caption{Quantitative comparison with competing methods in DISFA. }
\label{tab:disfa_all_criteria}
\end{table*}

% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{multirow}
% \begin{table}[]
% \begin{tabular}{@{}ccccccccccc@{}}
% \toprule
%  &
%   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Image\\ Category\end{tabular}} &
%   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Conditions\\ (Intensity)\end{tabular}} &
%   \multirow{2}{*}{} &
%   \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Image\\ Similarity\end{tabular}} &
%    &
%   \begin{tabular}[c]{@{}c@{}}Identity\\ Preservation\end{tabular} &
%    &
%   \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Editing\\ Accuracy\end{tabular}} \\ \cmidrule(lr){5-6} \cmidrule(lr){8-8} \cmidrule(l){10-11} 
%                                                                                 &                           &        &  & L2    & LPIPS &  & Distance &  & MSE   & ICC   \\ \midrule
% \multirow{4}{*}{DeltaEdit}                                                      & \multirow{2}{*}{Real}     & Target &  & 0.022 & 0.165 &  & 0.396    &  & 0.560 & 0.180 \\
%                                                                                 &                           & Zero   &  & -     & -     &  & -        &  & -     & -     \\ \cmidrule(l){2-11} 
%                                                                                 & \multirow{2}{*}{Inverted} & Target &  & 0.011 & 0.074 &  & 0.309    &  & 0.557 & 0.194 \\
%                                                                                 &                           & Zero   &  & -     & -     &  & -        &  & -     & -     \\ \midrule
% \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}ReDirTrans\\      -GAN\end{tabular}} & \multirow{2}{*}{Real}     & Target &  & 0.022 & 0.169 &  & 0.529    &  & 0.290 & 0.617 \\
%                                                                                 &                           & Zero   &  & 0.026 & 0.172 &  & 0.600    &  & 0.816 & -     \\ \cmidrule(l){2-11} 
%                                                                                 & \multirow{2}{*}{Inverted} & Target &  & 0.017 & 0.137 &  & 0.551    &  & 0.286 & 0.621 \\
%                                                                                 &                           & Zero   &  & 0.012 & 0.085 &  & 0.646    &  & 0.807 & -     \\ \cmidrule(l){2-11} 
% \multirow{4}{*}{AUEditNet (Ours)}                                               & \multirow{2}{*}{Real}     & Target &  & 0.026 & 0.174 &  & 0.468    &  & 0.283 & 0.628 \\
%                                                                                 &                           & Zero   &  & 0.026 & 0.179 &  & 0.426    &  & 0.102 & -     \\ \cmidrule(l){2-11} 
%                                                                                 & \multirow{2}{*}{Inverted} & Target &  & 0.016 & 0.126 &  & 0.435    &  & 0.281 & 0.630 \\
%                                                                                 &                           & Zero   &  & 0.016 & 0.098 &  & 0.383    &  & 0.100 & -     \\ \bottomrule
% \end{tabular}
% \end{table}
